Fluent Session Programming in C#

We propose SessionC#, a lightweight session typed library for safe concurrent/distributed programming. The key features are (1) the improved fluent interface which enables writing communication in chained method calls, by exploiting C#'s out variables, and (2) amalgamation of session delegation with async/await, which materialises session cancellation in a limited form, which we call session intervention. We show the effectiveness of our proposal via a Bitcoin miner application.

==> eptcsdata.tex <==
\providecommand{\firstpage}{61}
\providecommand{\publicationstatus}{S. Balzer, L. Padovani (Eds.): Programming Language Approaches\\
to Concurrency- \& Communication-cEntric Software (PLACES 2020)\\
EPTCS 314, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.314.6}{10.4204/EPTCS.314.6}}
\pdfoutput=1

